Contravariant pairings between standard Whittaker modules and Verma modules

We classify contravariant pairings between standard Whittaker modules and Verma modules over a complex semisimple Lie algebra. These contravariant pairings are useful in extending several classical techniques for category $\mathcal{O}$ to the Mili\v{c}i\'{c}--Soergel category $\mathcal{N}$. We introduce a class of costandard modules which generalize dual Verma modules, and describe canonical maps from standard to costandard modules in terms of contravariant pairings. We show that costandard modules have unique irreducible submodules and share the same composition factors as the corresponding standard Whittaker modules. We show that costandard modules give an algebraic characterization of the global sections of costandard twisted Harish-Chandra sheaves on the associated flag variety, which are defined using holonomic duality of $\mathcal{D}$-modules. We prove that with these costandard modules, blocks of category $\mathcal{N}$ have the structure of highest weight categories and we establish a BGG reciprocity theorem for $\mathcal{N}$.

==> old-stuff.tex <==





\section{Costandard Whittaker modules}
Let $M(\lambda,\eta)$ be a standard Whittaker module. Fix a contravariant form on $M(\lambda,\eta)$ corresponding to a Whittaker vector $w\in M(\lambda,\eta)^\ast$.
\begin{definition}
Let $M(\lambda,\eta)^{\vee_w}$ be the subspace of $M(\lambda,\eta)^\ast$ consisting of all locally $\n$-finite vectors $\phi$, for the $\eta$-twisted action of $\n$, such that 
\[
H^0_\eta(\n, U(\g)\phi)\subset \C w.
\]
\end{definition}
The subspace of locally $\n$-finite vectors is a $U(\g)$-submodule of $M(\lambda,\eta)^\ast$ (see Kostant Proposition 4.2.1). Moreover, because $U(\g)u\phi$ is a $U(\n)$-submodule of $U(\g)\phi$, for each $u\in U(\g)$ 
\[ H^0_\eta(\n, U(\g)u\phi)\subset H^0_\eta(\n, U(\g)\phi)\subset \C w.\]
Therefore, subspace of linear functions $\phi$ such that $H_\eta^0(\n,U(\g)\phi)\subset \C w$ is a $U(\g)$-module. This shows that $M(\lambda,\eta)^{\vee_w}$ is a $U(\g)$-module. 

% In the remaining sections of the paper we will calculate the $\eta$-twisted $\bar{\n}$-coinvariants of $U(\g)$-modules induced from $Z(\g)$-modules, and relate this space to the space of contravariant forms. 
% Let $\mathcal{J}_\eta$ be the right ideal in $U(\g)$ generated by $u-\eta(\tau(u))$ for each $u\in\bar{\n}$. Let $N_{U(\g)}\mathcal{J}_\eta$ be the normalizer of $\mathcal{J}_\eta$ in $U(\g)$,
% \[N_{U(\g)}\mathcal{J}_\eta = \{u\in U(\g) : [u,\mathcal{J}_\eta]\subset\mathcal{J}_\eta\}.  \]
% If $X$ is a $U(\g)$-module, then $H_0^\eta(\bar{\n},X)$ is naturally a $N_{U(\g)}\mathcal{J}_\eta$-module. 
% 
% \begin{problem}
% What is $N_{U(\g)}\mathcal{J}_\eta$? For any $\eta$, we have $Z(\g)\subset N_{U(\g)}\mathcal{J}_\eta$ and $\mathcal{J}_\eta\subset N_{U(\g)}\mathcal{J}_\eta$. If $\eta=0$, then we also have $U(\h)\subset N_{U(\g)}\mathcal{J}_\eta$. For $\g=\mathfrak{sl}_2$ and $\eta \neq 0$, $\frac{1}{2}h^2+h+2\eta x \in N_{U(\g)}\mathcal{J}_\eta$.
% \end{problem}








% \begin{proposition}
% The vector space of $\eta$-twisted $\bar{\n}$-coinvariants of $Y(\chi,\eta)$ is isomorphic to the space of $\bar{\n}$-coinvariants of $Y(\chi,\eta)$. 
% \end{proposition}
% \begin{proof}[Proof sketch.]
% The $\star$-action of $\bar{\n}$ on $Y(\chi,\eta)$ extends to a $\star$-action of $U(\bar{\n})$ on $Y(\chi,\eta)$ in the following way. If $x_1,x_2\in\bar{\n}$ and $y\in Y(\chi,\eta)$, then $(x_1x_2)\star y= x_1\star (x_2\star y)$. If $c\in \C$, let $cy=c\star y$. Since $U(\bar{\n})$ is generated by $\C$ and $\bar{\n}$, this defines a $\star$-action of $U(\bar{\n})$ on $Y(\chi,\eta)$. 

% The proof of the proposition follows from the statement: $Y(\chi,\eta)$ is a free $U(\bar{\n})$-module of rank $|W|$ with the $\star$-action of $U(\bar{\n})$. We will begin a proof of this statement with a short inductive argument, showing that given any $u\in U(\bar{\n})$, there exists a unique $u'\in U(\bar{\n})$ such that $uy=u'\star y$ for each $y \in Y(\chi,\eta)$. Fix an ordering of the negative roots: $\alpha_1,\cdots, \alpha_n\in -\Sigma^+$. Let $U(\bar{\n})_i$ denote the subspace of $U(\bar{\n})$ spanned by elements $x_{\alpha_1}^{d_1}\cdots x_{\alpha_n}^{d_n}$ such that $\sum_k d_k\le i$. Suppose $u\in U(\bar{\n})_0$ (i.e. $u\in \C$) and $y\in Y(\chi,\eta)$. Then 
% \[
% uy=u\star y .
% \]
% For the induction hypothesis we will assume that for each element $u\in U(\bar{\n})_{ n}$, there exists a unique element $u'\in U(\bar{\n})$ such that
% \[
% uy = u'\star y , 
% \]
% for all $y\in Y(\chi,\eta)$. 

% Suppose $u\in U(\bar{\n})_{n+1}$. Then we can write $u$ as a unique linear combination
% \[
% u = \sum_{j} c_jx^{I_j},
% \]
% where $c_j\in \C $, $I_j=\{d^j_1,\cdots, d^j_n\}\in \mathbb{Z}_{\ge 0}^n$, and $x^{I_j} = x_{\alpha_1}^{d^j_1}\cdots x_{\alpha_n}^{d^j_n}$. Let $m_j=\text{min}\{k: d_k\neq 0\}$ be the index corresponding to the first nonzero entry of $I_j=\{d^j_1,\cdots,d^j_n\}$. Let $x_j = x_{\alpha_{m_j}}$. Then $x^{I_j}=x_j x^{I'_j}$, and 
% \[
% u = \sum_{j} c_jx_j x^{I'_j}.
% \]
% Moreover, $x_j\in \bar{\n}$ and $x^{I'_j}\in U(\bar{\n})_{n}$. By the induction hypothesis, there exists a unique $u_j'\in U(\bar{\n})$ such that
% \[
% x^{I'_j} y = u_j'\star y. 
% \]
% Therefore 
% \begin{align*}
%     uy &= \sum_{j} x_j x^{I'_j} y\\
%     &= \sum_{j} x_j \cdot(u_j'\star y) \\
%     &= \sum_{j} (x_j-\eta(\tau(x_j)))\cdot(u_j'\star y )+\eta(\tau(x_j))\cdot(u_j'\star y)\\
%     &= \sum_{j} ((x_j + \eta(\tau(x_j)))u'_j)\star y\\
%     &= u'\star y,
% \end{align*}
% for $u'=\sum_{j}(x_j+\eta(\tau(x_j)))u_j'$. 
% Using Corollary \ref{free-module}, suppose $B$ is a basis of $Y(\chi,\eta)$ as a free $U(\bar{\n})$-module with the usual action of $U(\bar{\n})$. Any element $y\in Y(\chi,\eta)$ can be uniquely written as a linear combination 
% \[y=\sum_{b\in B}u_b b,\]
% with $u_b\in U(\bar{\n})$. Therefore, $y$ can be written uniquely as 
% \[y=\sum_{b\in B}u_b'\star  b.\]
% \end{proof}




% \begin{theorem}
% For any $\eta\in\ch\n$ and $\chi\in\ch Z(\g)$, 
% \[
% \dim \Psi = \dim H_0^\eta(\bar{\n},Y(\chi,\eta))^\ast = \dim H^0_\eta(\n, Y(\chi,\eta)^\ast)=|W|.
% \]
% \end{theorem}




 Clearly $w\in M(\lambda,\eta)^{\vee_w}$ is a Whittaker vector where $Z(\lev_\eta)$ acts by $\xi_\eta(\lambda)$. Any $U(\g)$-module morphism 
\[\varphi: M(\lambda,\eta)\rightarrow M(\lambda,\eta)^{\vee_w}, \]
must map $1\otimes 1$ to a Whittaker vector in $M(\lambda,\eta)^{\vee_w}$. The $U(\g)$-span of $\varphi(1\otimes 1)$ clearly contains the Whittaker vector $\varphi(1\otimes 1)$. Therefore $ \varphi(1\otimes 1)\in\C w$. This shows that 
\[ \Hom_{U(\g)}(M(\lambda,\eta),  M(\lambda,\eta)^{\vee_w}) \cong \C.\]
 Additionally, the kernel of such a map is the radical of the contravariant form on $M(\lambda,\eta)$ associated with $w$.
 \begin{proposition}
 $M(\lambda,\eta)^{\vee_w}$ decomposes into a direct sum of $\z$-weight spaces. Moreover, as $U(\lev_\eta)$-modules
 \[M(\lambda,\eta)^{\vee_w}_\mu\cong M(\lambda,\eta)_\mu. \] 
 This implies that in the Grothendieck group of $\N(\chi,\eta)$,
 \[
 [ M(\lambda,\eta)^{\vee_w}]=[M(\lambda,\eta)].
 \]
 \end{proposition}

==> sec-duality-general.tex <==
\section{Duality for Whittaker modules}
\label{duality for whittaker modules}

\begin{theorem}
For $X\in\N_\eta$ and $\mu\in\z^\ast$, let $X_\mu$ denote the generalized $\mu$-weight space of $X$ for the action of $\z$. Then $X_\mu$ is a Whittaker module over $\lev_\eta$. Moreover, $X$ decomposes as a direct sum of generalized $\z$-weight spaces. 
\end{theorem}
\begin{definition}
Let $\beta\in \C[W_\eta]$ be nonzero and $X\in \N_\eta$. Define
\[
X^{\vee_\beta}:=\bigoplus_\mu X_\mu^{\vee_\beta}. 
\]
\end{definition}
\begin{conjecture}
Suppose $X\in\N_\eta$ and $\beta\in\C[W_\eta]$ is nonzero. Then $X^{\vee_\beta}\in\N_\eta$ and $(X^{\vee_\beta})^{\vee_\beta}\cong X$. If $\eta=0$, then $X^{\vee_1}=X^\vee$ is the usual category $\mathcal{O}$ duality functor. 
\end{conjecture}
\begin{conjecture}
Fix a regular weight $\lambda\in\h^\ast$. Let $X$ be the flag variety of $\g$ and suppose $Q$ is an open $B$ orbit in a $P_\eta$ orbit on $X$. Let $\mathcal{O}_Q$ be an $\eta$-twisted $N$-equivariant connection on $Q$. Let $i$ be the inclusion map $i:Q\hookrightarrow X$. Fix a basis $\{\delta_w\}$ of $\C[W_\eta]$ and a $W_\eta$-equivariant isomorphism from $\C[W_\eta]$ to the $W_\eta$-coinvariants of $S(\h)$. Let $h_w$ be the image of $\delta_w$ under the fixed isomorphism. Let $\beta = \sum_{W_\eta} \lambda(h_w)\delta_w$. Then as $U(\g)$-modules,
\[
\Gamma(X,i_+\mathcal{O}_Q)^{\vee_\beta} \cong \Gamma(X, i_!\mathcal{O}_Q).
\]
More generally, if $\mathcal{M}$ is a holonomic $(\mathcal{D}_\lambda, N,\eta)$-module on $X$, then 
\[
\Gamma(X,\mathcal{M})^{\vee_\beta}\cong \Gamma(X,\mathbb{V}_X\mathcal{M}).
\]
\end{conjecture}

==> sec-duality-nondeg.tex <==
\section{Duality for nondegenerate Whittaker modules}
\label{duality for nondegenerate whittaker modules}

In this section we will outline a possible approach to an algebraic definition of duality for nondegenerate Whittaker modules. 


\begin{theorem}\cite{TwistedSheaves}
Let $\eta$ be nondegenerate. Then $I_\eta(\cdot)$ and $\Wh(\cdot)$ give an equivalence of categories between $\mathcal{Z}_\g$ and $\N_\eta$.  
\end{theorem}
Given $\beta\in \C[W]$ and $\varphi\in U^\ast$, define
\begin{align*}
    \phi_{\beta,\varphi}:H_0^\eta(\bar{\n},I_\eta(U))&\rightarrow \C,\\
    1\otimes b_w\otimes v&\mapsto \beta(w)\varphi(v)
\end{align*}
and 
\begin{align*}
    \Phi^U_\beta: I_\eta(U^\ast)&\rightarrow (I_\eta(U))^\ast\\
    u\otimes \varphi &\mapsto u\cdot \phi_{\beta,\varphi}
\end{align*}
where we view $\phi_{\beta, \varphi}$ as a Whittaker vector in $(I_\eta(U))^\ast$. 
\begin{conjecture}
If $\eta$ is nondegenerate, then $\Phi^U_\beta$ is an injective morphism of $U(\g)$-modules for all nonzero $\beta\in\C[W]$ and all $U\in\mathcal{Z}_\g$. 
\end{conjecture}
\begin{definition}
Let $\eta$ be nondegenerate. Then for each $X\in \N_\eta$ we have
\[ X \cong I_\eta( \text{Wh}(X)).\]
For $\beta\in\C[W]$ nonzero, define
\[ X^{\vee_\beta} := \im  \Phi^{\Wh(X)}_\beta. \]

\end{definition}




==> sec-forms-on-induced.tex <==
\section{Contravariant forms on $U(\g)$-modules induced from $Z(\g)$-modules}
\label{contravariant forms on U(g)-modules induced from Z(g)-modules}




Let $\mathcal{Z}_\g$ denote the category of finite dimensional $Z(\g)$-modules. Let $U$ be a finite dimensional $Z(\g)$-module. For $\eta\in\ch U(\n)$, let $U_\eta$ denote the $Z(\g)\otimes U(\n)$-module $ U\otimes_\C \C_\eta$. Define the functor $I_\eta$ from $\mathcal{Z}_\g$ to $\N_\eta $ by
\[
I_\eta(U):= U(\g)\otimes_{Z(\g)\otimes U(\n)}U_\eta.
\]
In this section we will give a classification of contravariant forms on all $U(\g)$-modules of the form $I_\eta(U)$, for some $U\in\mathcal{Z}_\g$. 

We begin by computing the dimension of $\eta$-twisted $\bar{\n}$-coinvariants of $I_\eta(U)$, using Theorem \ref{U-free}. 
\begin{theorem}{\label{free-module}}
As $Z(\g)$-modules
\[
    H_0^\eta(\bar{\n},I_\eta(U))\cong \bigoplus_W U.
\]
Moreover,
\[
\dim H_0^\eta(\bar{\n},I_\eta(U)) = |W|\cdot\dim U.
\]
\end{theorem}
\begin{proof}
By definition, 
\[
 H_0^\eta(\bar{\n},I_\eta(U)) = \C_{\bar{\eta}}\otimes_{U(\bar{\n})} U(\g)\otimes_{Z(\g)\otimes U(\n)} U_\eta, 
\]
where $U(\g)$ is viewed as a $(U(\bar{\n}),Z(\g)\otimes U(\n))$-bimodule, $U_\eta$ a left $Z(\g)\otimes U(\n)$-module, and $\C_{\bar{\eta}}$ a right $U(\bar{\n})$-module.
By Conjecture \ref{U-free}, $U(\g)$ is a free $ U(\bar{\n})\otimes (Z(\g)\otimes U(\n))^{\text{op}}$-module of rank $|W|$. Therefore, if $\{b_w\}_{w\in W}$ is a basis for $U(\g)$ as a $ U(\bar{\n})\otimes (Z(\g)\otimes U(\n))^{\text{op}}$-module, and $\{e_j\}_{j\in J}$ is a basis for $U_\eta$ (as a vector space), then $\{ 1\otimes b_w\otimes e_j\}_{(w,j)\in   W\times J}$ is a basis for $ H_0^\eta(\bar{\n},I_\eta(U))$ (as a vector space). The action of $z\in Z(\g)$ on $1\otimes b_w\otimes e_j$ is given by
\[z\cdot(1\otimes b_w\otimes e_j)=1\otimes zb_w\otimes e_j =1\otimes b_w\otimes ze_j, \]
since $[z,b_w]=0$. Therefore, 
$\bigoplus_J \C (1\otimes b_w\otimes e_j)$ is a $Z(\g)$-module isomorphic to $U$. 
\end{proof}

\begin{example}
Suppose $\eta\in\ch\n$ is nondegenerate. Then $I_\eta(\mathbb{C}_{\chi}) = Y(\chi,\eta)$ is an irreducible Whittaker module, and
\[  H_0^\eta(\bar{\n},Y(\chi,\eta))\cong  \bigoplus_W\C_\chi . \]
\end{example}
\begin{example}
Suppose $\eta=0$. Then $H_0^\eta(\bar{\n},I_\eta(U))$ is a $U(\h)$-module, since $ Z(\lev_\eta)= U(\lev_\eta)=U(\h)$. Suppose $\chi\in\ch Z(\g)$ is regular and corresponds to the $W$ orbit of $\lambda\in\h^\ast$. Then $I_\eta(\mathbb{C}_{\chi}) = Y(\chi,\eta) = \bigoplus_W M(w\cdot\lambda)$ is a direct sum of Verma modules \cite[Corollary 2.5]{CompositionSeries}, and
\[   H_0^\eta\left(\bar{\n},\bigoplus_W M(w\cdot\lambda)\right)= \bigoplus_W \C_{w\cdot\lambda} . \]
If $\eta=0$ and $\chi\in\ch Z(\g)$ is singular, then $I_\eta(\C_\chi)$ admits a filtration with subquotients $M(w\cdot\lambda)$, where $w$ runs over $W$ \cite[Corollary 2.5]{CompositionSeries}. 

Notice that because the $\bar{\n}$-coinvariants functor $H_0(\bar{\n},\cdot):\mathcal{O}'\rightarrow U(\h)\text{-mod}$ is not exact, it is not necessarily true that in the $K$-group of $U(\h)$-mod, $[H_0(\bar{\n},X)]$ is equal to $ \sum_{\mu\in\Lambda} [\C_{\mu}]$ for any module $X$ with a filtration consisting a subquotients isomorphic to $M(\mu)$, for various $\mu\in \Lambda$. However, we have shown that 
\[
  H_0^\eta(\bar{\n},I_\eta(\C_\chi)) = \bigoplus_W \C_\chi. 
\]
Therefore, the generalized weights of $ H_0^\eta(\bar{\n},I_\eta(\C_\chi)) $ must lie in the $W$ orbit of $\lambda$, and $\dim H_0^\eta(\bar{\n},I_\eta(\C_\chi)) =|W|$.
\begin{problem}
Show that as $U(\h)$-modules
\[   H_0\left(\bar{\n},I_{\eta=0}(\C_\chi)\right)= \bigoplus_W \C_{w\cdot\lambda} \]
for singular $\chi$. 
\end{problem}
\end{example}
\begin{theorem}
$H_0^\eta(\bar{\n},X)$ is a $Z(\lev_\eta)$-module for each $U(\g)$-module $X$, and the functor 
\begin{align*}
    H_0^\eta(\bar{\n},I_\eta(\cdot)):\mathcal{Z}_\g\rightarrow \mathcal{Z}_{\lev_\eta}
\end{align*}
is exact. 
{\color{red}{The next statement still needs a proof.}}
Let $\phi$ be the PBW projection map $\phi:U(\g)\rightarrow U(\lev_\eta)$. Then the restriction of $\phi$ to $Z(\g)$ is an injection from $Z(\g)$ into $Z(\lev_\eta)$. We will use $\phi$ to view $Z(\lev_\eta)$ as a $Z(\g)$-module. As $Z(\lev_\eta)$-modules
\[
H_0^\eta(\bar{\n},I_\eta(U))\cong \bigoplus_{W_\eta}Z(\lev_\eta)\otimes_{Z(\g)} U. 
\]
\end{theorem}
\begin{proof}
We will begin by showing that $H_0^\eta(\bar{\n},X)$ is a $Z(\lev_\eta)$-module. Let $\p_\eta$ be the parabolic subalgebra of $\g$ determined by $\Pi_\eta:=\{\alpha\in\Pi:\eta\vert_{\g_\alpha}\neq 0\}$ and $\bar{\p}_\eta = \tau(\p_\eta)$. Then $\bar{\n}^\eta:=[\bar{\p}_\eta,\bar{\p}_\eta]$ is an ideal in $\bar{\p}_\eta$. Let $\bar{\p}_\eta=\lev_\eta\oplus\bar{ \n}^\eta$ and $\bar{\n}_\eta =\bar{\n}\cap\lev_\eta$. Then $\bar{\n}=\bar{\n}_\eta\oplus\bar{\n}^\eta$. Since $\bar{\n}^\eta$ is an ideal in $\bar{\p}_\eta$, 
\[ [\lev_\eta,\bar{\n}^\eta]\subset \bar{\n}^\eta.\]
Therefore, if $X$ is a $U(\g)$-module, then $U(\lev_\eta)\cdot \bar{\n}^\eta X \subset \bar{\n}^\eta X$. Therefore, the space of $\bar{\n}^\eta$-coinvariants of $X$, $X/ \bar{\n}^\eta X$, is a $U(\lev_\eta)$-module. Moreover, if $u\in\bar{\n}^\eta$, then $\eta(\tau(u))=0$. Therefore, the $\star$ action of $\n^\eta$ agrees with the usual action of $\n^\eta$. Therefore, the space of $\eta$-twisted $\bar{\n}^\eta$-coinvariants of $X$ is naturally a $U(\lev_\eta)$-module. 

By definition, $[Z(\lev_\eta),\bar{\n}_\eta]=0$, since $\bar{\n}_\eta\in U(\lev_\eta)$. Therefore, \[z\cdot (u-\eta(\tau(u))) = (u-\eta(\tau(u)))z,\] for each $z\in Z(\lev_\eta)$ and $u\in\bar{\n}_\eta$. This shows that 
\[
z\cdot \bar{\n}_\eta\star X\subset \bar{\n}_\eta\star X, 
\]
for each $z\in Z(\lev_\eta)$. Therefore, the space of $\eta$-twisted $\bar{\n}_\eta$-coinvariants is a $Z(\lev_\eta)$-module. 

Since $\bar{\n}=\bar{\n}_\eta\oplus\bar{\n}^\eta$, for each $U(\g)$-module $X$, we have 
\begin{align*}
    z\cdot \bar{\n}\star X &= z\cdot (\bar{\n}_\eta\star X\oplus \bar{\n}^\eta\star X)\\
    &= z\cdot\bar{\n}_\eta\star X \oplus z\cdot \bar{\n}^\eta\star X\\
     &\subset \bar{\n}_\eta\star X \oplus  \bar{\n}^\eta\star X\\
    &\subset \bar{\n}\star X, 
\end{align*}
for all $z\in Z(\lev_\eta)$. Therefore, the space of $\eta$-twisted $\bar{\n}_\eta$-coinvariants of a $U(\g)$-module $X$ is naturally a module over $Z(\lev_\eta)$. 

{\color{red} Next we want to try to find a concrete description of $H_0^\eta(\bar{\n},I_\eta(U))$ as a $Z(\lev_\eta)$-module. The following is a sketch of an idea for a proof.}

Notice that $\eta$ is trivial when restricted to $\n^\eta$. Therefore 
\[
\C_{\bar{\eta}}\otimes_{U(\bar{\n})}U(\g)\otimes_{Z(\g)\otimes U(\n)} U = \C_{\bar{\eta}}\otimes_{U(\bar{\n}^\eta)}U(\lev_\eta)\otimes_{Z(\g)\otimes U(\n^\eta)} U,
\]
where $U(\lev_\eta)$ is a $Z(\g)$-module by the PBW projection $\phi:U(\g)\rightarrow U(\lev_\eta)$. We can apply Theorem \ref{U-free} to $U(\lev_\eta)$ to get a basis, indexed by $W_\eta$, for $U(\lev_\eta)$ as a $(U(\bar{\n}_\eta),Z(\lev_\eta)\otimes U(\n_\eta))$-bimodule. Therefore, every vector in $U(\lev_\eta)$ can be written as a unique linear combination of elements of the form $yb_w zx$ with $y\in U(\bar{\n}^\eta)$, $b_w$ a basis element, $z\in Z(\lev_\eta)$, and $x\in U(\n^\eta)$. This shows that every element in $H_0^\eta(\bar{\n}, I_\eta(U))$ is a linear combination of elements of the form 
\[
1\otimes b_wz\otimes u,
\]
for $z\in Z(\lev_\eta)$ and $u\in U$. The action of $Z(\lev_\eta)$ on this vector space is given by multiplication on the middle term of simple tensors. Because $Z(\lev_\eta)$ commutes with $b_w$, the space 
\[\C_\eta\otimes b_w Z(\lev_\eta)\otimes_{Z(\g)} U\]
is a $Z(\lev_\eta)$-submodule of $\C_{\bar{\eta}}\otimes_{U(\bar{\n})}U(\g)\otimes_{Z(\g)\otimes U(\n)} U$, which is isomorphic to 
\[
Z(\lev_\eta)\otimes_{Z(\g)}U. 
\]
{\color{red} The isomorphism part of the previous statement needs justification.} Moreover, the space $\C_\eta\otimes b_w Z(\lev_\eta)\otimes_{Z(\g)} U$ is orthogonal to $\C_\eta\otimes b_y Z(\lev_\eta)\otimes_{Z(\g)} U$ for $b_w\neq b_y$, because $Z(\lev_\eta)$ acts freely on $b_w$ and $b_y$ ({\color{red} again, this needs more justification}). Finally, fixing an isomorphism for each basis element $b_w$, the resulting map
\begin{align*}
  \C_{\bar{\eta}}\otimes_{U(\bar{\n})}U(\g)\otimes_{Z(\g)\otimes U(\n)} U  &\rightarrow  \bigoplus_{w\in W_\eta} Z(\lev_\eta)\otimes_{Z(\g)}U
\end{align*}
is an isomorphism of $Z(\lev_\eta)$-modules. 
\end{proof}
We will now relate $\eta$-twisted $\bar{\n}$-coinvariants on $Y(\chi,\eta)$ to contravariant forms on $Y(\chi,\eta)$. First we will recall \cite[Proposition 3.2]{BrownRomanov} and \cite[Proposition 3.5]{BrownRomanov}. 

\begin{conjecture}
{\color{red}This is probably not true... $Z(\g)$ is not a PID for $\g$ rank $>1$} Every finite dimensional $Z(\g)$-module is isomorphic to a direct sum of cyclic $Z(\g)$-modules. Moreover, every module of the form $I_\eta(U)$ is isomorphic to a direct sum of cyclic $U(\g)$-modules. 
\end{conjecture}


\begin{proposition}\cite[Proposition 3.2]{BrownRomanov}
\label{forms-functionals}
The set of contravariant forms on a cyclic $U(\g)$-module $X=U(\g)v$ are in bijection with linear functionals $\varphi:U(\g)\rightarrow \mathbb{C}$ satisfying the following conditions:
\begin{enumerate}[(a)]
\item $\varphi\left(\text{Ann}_{U(\g)}v\right)=0$, and 
\item $\varphi(u)=\varphi(\tau(u))$ for all $u \in U(\g)$.
\end{enumerate}
\end{proposition}
\begin{proposition}\cite[Proposition 3.5]{BrownRomanov}
\label{first Ug decomp} Let $\eta:\mf{n}\rightarrow \C$ be a Lie algebra morphism and $\ker{\eta}\subset U(\n)$. There is a direct sum decomposition
\begin{equation}
    \label{twisted HC hom}
    U(\g)=U(\h)\oplus (\tau(U(\mf{g})\ker{\eta})+U(\g)\ker{\eta}).
\end{equation}
\end{proposition}

\begin{proposition}
The space of contravariant forms on $Y(\chi,\eta)$ is isomorphic to the space of linear functionals on $ H_0^\eta(\bar{\n},Y(\chi,\eta))$. 
\end{proposition}
\begin{proof}
Let $w=1\otimes 1\in Y(\chi,\eta)$. Given a contravariant form $\langle,\rangle$ on $Y(\chi,\eta)$, define a linear functional on $Y(\chi,\eta)$ as follows:
\[\phi_{\langle,\rangle}(y)=\langle y, w\rangle.  \]
If $y\in \bar{\n}\star Y(\chi,\eta)$, then $y=(u-\eta(\tau(u)))y'$ for some $u\in \bar{\n}$ and $y'\in Y(\chi,\eta)$. Then it follows that 
\[\phi_{\langle,\rangle}(y)=\langle (u-\eta(\tau(u)))y', w\rangle=\langle y', (\tau(u)-\eta(\tau(u)))w\rangle = 0 ,\]
because $\tau(u)-\eta(\tau(u))$ annihilates $w$. Therefore $\phi_{\langle,\rangle}$ vanishes on $\bar{\n}\star Y(\chi,\eta)$. So the linear functional $\phi_{\langle,\rangle}$ factors through the quotient 
\begin{center}
\begin{tikzpicture}[scale=1.5]
\node at (0,0) {$Y(\chi,\eta)$};
\node at (0,-1) {$Y(\chi,\eta)/\bar{\n}\star Y(\chi,\eta)$};
\node at (3,-1) {$\C$};
\draw[->](0,-.2)--(0,-.8) node[midway,left] {$q$};
\draw[->](.5,-.1)--(2.8,-.9)node[midway,above] {$\phi_{\langle,\rangle}$};
\draw[->](1,-1)--(2.8,-1)node[midway,below] {$\bar{\phi}_{\langle,\rangle}$};
\end{tikzpicture}
\end{center}
Therefore we have a map from $\Psi$, the space of contravariant forms on $Y(\chi,\eta)$, to $H_0^\eta(\bar{n},Y(\chi,\eta))^\ast$:
\begin{eqnarray*}
\Psi&\rightarrow & H_0^\eta(\bar{n},Y(\chi,\eta))^\ast.\\
\langle,\rangle&\mapsto& \bar{\phi}_{\langle,\rangle}
\end{eqnarray*}
We will complete the proof by constructing an inverse of the above linear map. Suppose $\gamma\in H_0^\eta(\bar{n},Y(\chi,\eta))^\ast$. Define a linear functional $\tilde{\gamma}$ on $U(\g)$ by 
\[\tilde{\gamma}(u):=\gamma(q(uw)).\]
We aim to use Proposition \ref{forms-functionals} to identify a contravariant form $\langle,\rangle_\gamma$ with the linear functional $\tilde{\gamma}\in U(\g)^\ast$. In order to make this association, we need to check that $\tilde{\gamma}$ vanishes on $\Ann_{U(\g)}w$ and $\tilde{\gamma}$ is $\tau$-invariant. By definition $\tilde{\gamma}(\Ann_{U(\g)})=0$. We can check the $\tau$-invariance of $\tilde{\gamma}$ by applying Proposition \ref{first Ug decomp}. If $x\in \ker\eta$, then $\tilde{\gamma}(ux)=0$, because $ux\in \Ann_{U(\g)}w$. If $y\in \tau(\ker\eta)$, then $\tilde{\gamma}(yu)=\gamma(q(yuw))=0$ because $yuw\in \bar{\n}\star Y(\chi,\eta)$. Therefore $\tilde{\gamma}$ vanishes on $\tau(U(\g)\ker\eta)+U(\g)\ker\eta$. Using Proposition \ref{first Ug decomp}, write $u\in U(\g)$ as $u=h+x$, where $h\in U(\h)$ and $x\in \tau(U(\g)\ker\eta)+U(\g)\ker\eta$. Notice that $\tau(u)=h+\tau(x)$. We have that
\begin{align*}
\tilde{\gamma}(u)&=\tilde{\gamma}(h+x)\\
&=\tilde{\gamma}(h)\\
&=\tilde{\gamma}(h+\tau(x))\\
&=\tilde{\gamma}(\tau(u)).
\end{align*}
Finally, we can easily check that the linear map 
\begin{align*}
\varphi:H_0^\eta(\bar{n},Y(\chi,\eta))^\ast&\rightarrow \Psi\\
\gamma&\mapsto \langle ,\rangle_{\tilde{\gamma}}
\end{align*}
is the inverse of 
\begin{align*}
\psi:\Psi&\rightarrow  H_0^\eta(\bar{n},Y(\chi,\eta))^\ast,\\
\langle,\rangle&\mapsto \bar{\phi}_{\langle,\rangle}
\end{align*}
by showing that $(\psi\circ\varphi)(\gamma)=\gamma$:
\begin{align*}
  \left(\psi\circ\varphi(\gamma)\right)(y+\bar{\n}\star Y(\chi,\eta))&=  \bar{\phi}_{\langle,\rangle_{\tilde{\gamma}} } (y+\bar{\n}\star Y(\chi,\eta))\\
  &= \langle y,w\rangle_{\tilde{\gamma} }\\
    &= \gamma(q(y))\\
    &= \gamma(y+\bar{\n}\star Y(\chi,\eta)). 
\end{align*}

\end{proof}

\begin{proposition}
 $H_0^\eta(\bar{\n},Y(\chi,\eta))^\ast$ is canonically isomorphic to the space of Whittaker vectors in $Y(\chi,\eta)^\ast$: 
\begin{align*}
    H_0^\eta(\bar{\n},Y(\chi,\eta))^\ast&\rightarrow H^0_\eta(\n, Y(\chi,\eta)^\ast).\\
    \gamma&\mapsto \gamma\circ q
\end{align*}
\end{proposition}
\begin{proof}
We can check that this map is well-defined by showing that $\gamma\circ q $ is annihilated by the $\eta$-twisted action of $\n$:
\[ (u-\eta(u))(\gamma\circ q)(y)=\gamma(q((\tau(u)-\eta(u))y))=0\]
for $u\in \n$ and $y\in Y(\chi,\eta)$, because $(\tau(u)-\eta(u))y\in \bar{\n}\star Y(\chi,\eta)$. Hence $\gamma\circ q$ is a Whittaker vector in $Y(\chi,\eta)^\ast$. To see that this map is an isomorphism, we can check that each Whittaker vector in $Y(\chi,\eta)^\ast$ factors through the quotient map $q$. Suppose $\phi\in H^0_\eta(\n, Y(\chi,\eta)^\ast)$. Then 
\[ \phi(u\star y) = \phi((u-\eta(\tau(u)))y) = \tau(u)\phi(y)-\eta(\tau(u))\phi(y) = 0 \]
for $u\in \bar{\n}$ and $y\in Y(\chi,\eta)$. This shows that each Whittaker vector $\phi \in H^0_\eta(\n, Y(\chi,\eta)^\ast)$ vanishes on the subspace $\bar{\n}\star Y(\chi,\eta)$ of $Y(\chi,\eta)$. Therefore $\phi$ factors through the quotient map $q$:
\begin{center}
\begin{tikzpicture}[scale=1.5]
\node at (0,0) {$Y(\chi,\eta)$};
\node at (0,-1) {$Y(\chi,\eta)/\bar{\n}\star Y(\chi,\eta)$};
\node at (3,-1) {$\C$};
\draw[->](0,-.2)--(0,-.8) node[midway,left] {$q$};
\draw[->](.5,-.1)--(2.8,-.9)node[midway,above] {$\phi$};
\draw[->](1,-1)--(2.8,-1)node[midway,below] {$\bar{\phi}$};
\end{tikzpicture}
\end{center}
Altogether, we have shown that for each $\phi \in  H^0_\eta(\n, Y(\chi,\eta)^\ast)$ there is a $\bar{\phi}\in H_0^\eta(\bar{\n},Y(\chi,\eta))^\ast$ such that $\phi= \bar{\phi}\circ q$. 
\end{proof}
\begin{conjecture}
Let $\Psi_{I_\eta(U)}$ denote the vector space of contravariant forms on $I_\eta(U)$. Then there are linear isomorphisms
\[
\Psi_{I_\eta(U)}\cong (H_0^\eta(\bar{\n},I_\eta(U)))^\ast\cong H^0_\eta(\n,(I_\eta(U))^\ast).
\]
\end{conjecture}

==> sec-free-bimodule.tex <==
\section{The universal enveloping algebra as a free bimodule}
\label{the universal enveloping algebra as a free bimodule}

\begin{definition}
We say that a $(R,S)$-bimodule $M$ is a \emph{free $(R,S)$-bimodule of rank $n$} if $M$ is a free $R\otimes S^{\text{op}}$-module of rank $n$. 
\end{definition}

\begin{theorem}\label{U-free}
$U(\g)$ is a free $(U(\bar{\n}),Z(\g)\otimes U(\n))$-bimodule of rank $|W|$. 
\end{theorem}
\begin{proof}
Following the proof of Lemma 5.7 in \cite{TwistedSheaves}. Let $\{U_p(\g);p\in\mathbb{Z}_{\ge 0}\}$ denote the filtration of $U(\g)$ induced from the degree filtration of PBW basis elements. Let $F_pU(\g)$ be the linear filtration of $U(\g)$ defined by 
\[F_pU(\g)=U(\bar{\n})\otimes_\C U_p(\h)\otimes_\C U(\n).\]
The $F_p$ filtration of $Z(\g)\otimes U(\n)$ (viewed as a subspace of $U(\g)$) is related to the natural $U_p(\g)$ filtration of $U(\g)$ by 
\[
F_p(Z(\g)\otimes U(\n))=(U_p(\g)\cap Z(\g))\otimes U(\n). 
\]
The $F_p$ filtration of $Z(\g)\otimes U(\n)$ preserves the ring structure of $Z(\g)\otimes U(\n)$, i.e. if $u\in F_p(Z(\g)\otimes U(\n))$ and $u'\in F_q(Z(\g)\otimes U(\n))$, then $uu'\in F_{p+q}(Z(\g)\otimes U(\n))$. Therefore, the corresponding graded object $\text{gr}(Z(\g)\otimes U(\n))$ is a ring. Moreover, as rings, 
\[
\text{gr}(Z(\g)\otimes U(\n))\cong \text{gr}Z(\g)\otimes U(\n),
\]
where $\text{gr}Z(\g)$ denotes the graded ring associated to the filtration $U_p(\g)\cap Z(\g)$ of $Z(\g)$. It is well-known that the Harish-Chandra homomorphism $\gamma$ preserves the filtrations of $Z(\g)$ and $S(\h)$, and induces an isomorphism $\text{gr}\gamma$ from $\text{gr}Z(\g)$ to $S(\h)^W$. 

Suppose $z\in F_p(Z(\g))$. Then the Harish-Chandra homomorphism implies $z-\gamma(z)\in U_{p-1}(\g)\n$ and $\gamma(z)\in U_p(\h)$. Viewing $U(\g)$ as a right $Z(\g)\otimes U(\n)$-module, we have
\begin{align*}
U_q(\h)\cdot z &\subset  U_q(\h)\gamma(z)+U_q(\h)U_{p-1}(\g)\n \\
& \subset U_{q+p}(\h)+U_{q+p-1}(\g)\n\\
&\subset U_{q+p}(\h)+F_{q+p-1}U(\g) \subset F_{q+p}U(\g),
\end{align*}
because $U_{q+p-1}(\g)\subset F_{q+p-1}U(\g)$ and $\n\in F_0U(\g)$. This implies that $U(\g)$ is a filtered right $Z(\g)\otimes U(\n)$-module. Suppose $u\in U(\bar{\n})$. Then
\begin{align*}
    u\cdot F_pU(\g)&\subset u\cdot (U(\bar{\n})\otimes_\C U_p(\h)\otimes_\C U(\n))\\
    &\subset  F_pU(\g).
\end{align*}
Therefore, the left action of $U(\bar{\n})$ on $U(\g)$ preserves the $F_pU(\g)$ filtration of $U(\g)$. Altogether, we have shown that $U(\g)$ is a filtered $(U(\bar{\n}),Z(\g)\otimes U(\n))$-bimodule. 


Let $\text{gr}U(\g)$ denote the graded $(U(\bar{\n}),\text{gr}Z(\g)\otimes U(\n))$-bimodule corresponding to the $F_pU(\g)$ filtration of $U(\g)$. We have that 
\[\text{gr}U(\g)\cong U(\bar{\n})\otimes_\C U(\h)\otimes_\C U(\n),\] 
where $U(\bar{\n})$ acts by left multiplication, $\text{gr}Z(\g)=S(\h)^W$ acts on the $U(\h)$ factor, and $U(\n)$ acts by right multiplication. It is well-known that $U(\h)$ is a free $S(\h)^W$-module of rank $|W|$. Moreover, as $\C[W]$-modules, 
\[
U(\h)\cong \C[W]\otimes_\C S(\h)^W. 
\]
Therefore, $\text{gr}U(\g)$ is a free $(U(\bar{\n}),\text{gr}Z(\g)\otimes U(\n))$-bimodule of rank $|W|$. Let $\{\delta_w:w\in W\}$ be the canonical vector space basis for $\C[W]$, and identify each $\delta_w$ with an element $b_w$ of $U(\h)$ using the above isomorphism. Then \[\{1\otimes b_w\otimes 1 \in U(\bar{\n})\otimes_\C U(\h)\otimes_\C U(\n):w\in W\}\]
is a basis of $\text{gr}U(\g)$ as a free $(U(\bar{\n}),Z(\g)\otimes U(\n))$-bimodule. It follows that $U(\g)$ is a free $(U(\bar{\n}),Z(\g)\otimes U(\n))$-bimodule of rank $|W|$, with basis given by $\{b_w\}$. {\color{red} Notice that there is a natural filtration of basis elements $\{b_w\}$ induced by the filtrations of $U(\g)$ (the $F_p$ and the natural filtration should agree on each $b_w$). This suggests that even in the nondegenerate setting, we can possible distinguish different contravariant forms by their degree. }

\end{proof}

==> sec-functors.tex <==
\section{Duality Functors}
\label{duality functors}

In this section we introduce a family of duality functors between blocks of $\N$. 
\begin{lemma}
Each object in $\N$ is finitely generated over $U(\bar{\n})$. 
\end{lemma}
\begin{proof}
Objects in $\N$ are finitely generated over $U(\g)$,  locally $U(\n)$-finite, and locally $Z(\g)$-finite.  Therefore, for $v\in X\in \N$, $(Z(\g)\otimes U(\n))\cdot v$ is finite dimensional. By Lemma \ref{U-free}, $U(\g)$ is a finitely generated free $(U(\bar{\n}),Z(\g)\otimes U(\n))$-bimodule. Therefore, $U(\g)v$ is finitely generated as a left $U(\bar{\n})$-module. The result follows from the assumption that $X$ is finitely generated as a $U(\g)$-module.
\end{proof}
\begin{proposition}
Let $\eta\in\ch\n$. The functor defined by
\begin{align*}
    \nabla_\eta: \N&\rightarrow \N(\eta)\\
    X&\mapsto (X^\ast)_\eta,
\end{align*}
is an exact contravariant functor. 
Recall that $(X^\ast)_\eta$ denotes the $\eta$-twisted $U(\n)$-finite vectors in $X^\ast$. 
\end{proposition}
\begin{proof}
This should follow from the fact that objects in $\N$ are finitely generated over $U(\bar{\n})$ and \cite[Lemma 4.5]{Kostant}. 
\end{proof}
\begin{remark}
Notice that the restriction of $\nabla_0$ to $\cO$ is the category $\cO$ contravariant duality functor $\cO \xrightarrow{\vee} \cO $. 
\end{remark}
\begin{proposition}\label{prop:translation-standard}
Let $\lambda$ be $\n_\eta$-dominant. Then
\[
\nabla_0(M(\lambda,\eta))\cong M^\vee(\lambda). 
\]
\end{proposition}
\begin{definition}
The \emph{contravariant duality functor} $\vee:\N(\eta)\rightarrow \N(\eta)$
is defined by
\[
X^\vee: = \nabla_\eta\circ \nabla_0\circ \nabla_0 (X). 
\]

\end{definition}

\begin{remark}
Notice that the composition of functors $\nabla_\eta\circ\nabla_0$ is isomorphic to Backelin's functor: $\overline{\Gamma}_\eta(X) := \overline{X}_\eta$. 
\end{remark}
\begin{proposition}
Let $\eta\in\ch\n$ and $\mu\in\z^\ast$. Then projection onto a $\z$-weight space defines an exact functor 
\begin{align*}
    (\cdot)_\mu:\N_\g&\rightarrow \N_{\lev_\eta}.
\end{align*}
\end{proposition}
We will abuse notation and use $\nabla_\eta$ to denote the functor $\nabla_\eta(X)= (X^\ast)_\eta$ for modules $X$ in $\N_{\lev_\eta}$ as well as for modules $X$ in $\N_\g$. 
\begin{lemma}
Let $X\in\cO$, $\eta\in\ch\n$, and $\mu\in \z^\ast$. Then 
\[
\left(\nabla_\eta X\right)_\mu \cong \nabla_\eta\left(X_\mu\right)
\]
as $\lev_\eta$-modules.
\end{lemma}
\begin{lemma}
Let $X\in\N(\eta)$ and $\mu\in\z^\ast$. Then
\[
(\nabla_0 X)_\mu \cong \nabla_0(X_\mu)
\]
as $\lev_\eta$-modules. 
\end{lemma}
\begin{proposition}
Let $X\in\N(\eta)$ and $\mu\in\z^\ast$. Then
\[
(X_\mu)^\vee \cong (X^\vee)_\mu
\]
as $\lev_\eta$-modules. 
\end{proposition}
\begin{lemma}
Let $\eta\in\ch\n$ be nondegenerate. Then
\begin{enumerate}
    \item $Y(\lambda,\eta)^\vee\cong Y(\lambda,\eta)$ and 
    \item $(X^\vee)^\vee\cong X$ for all $X\in\N(\eta)$. 
\end{enumerate}
\end{lemma}
\begin{lemma}
The functor
\[
\nabla_\eta\circ\nabla_0:\N(\eta)\rightarrow\N(\eta)
\]
is isomorphic to the identity functor. 
\end{lemma}
\begin{theorem}
Let $\eta\in\ch\n$ and $\lambda$ be regular and $\n_\eta$-dominant. The duality functor on $\N(\eta)$ is exact, contravariant, and has the following properties: 
\begin{enumerate}
    \item $\left(M(\lambda,\eta)\right)^\vee = M_1^\vee(\lambda,\eta)$, 
    \item $X^\vee \cong X$ for $X$ irreducible, and
    \item $(X^\vee)^\vee \cong X$ for all $X\in\N(\eta)$.
\end{enumerate}
\end{theorem}
\begin{proof}[Proof Sketch.]
By Proposition \ref{prop:translation-standard}, $\nabla_0(M(\lambda,\eta))\cong M^\vee(\lambda)$. Using duality for category $\cO$, we have
\[
\nabla_0(M^\vee(\lambda)) = M(\lambda),
\]
which implies (1). 


\end{proof}

\begin{corollary}
The contravariant duality functor lifts to a stratified equivalence of categories of $D$-modules, which interchanges $*$-standard and $!$-standard objects. 
\end{corollary}

==> sec-outline.tex <==
Outline:
\begin{enumerate}
    \item Introduction
    \begin{enumerate}
        \item In $\cO$, contravariant forms correspond to canonical maps of $D$-modules
        \item For Whittaker modules in general, contravariant forms are not unique, not easy to see how they relate to canonical maps 
        \item In this paper we give an algebraic interpretation of the canonical map and costandard modules in a way which generalized classical results for $\cO$
    \end{enumerate}
    \item Algebraic Preliminaries
    \begin{enumerate}
        \item Category of Whittaker modules
        \item Kostant results
        \item McDowell results
        \item Backelin results
        \item Lie algebra homology definition
    \end{enumerate}
    \item Geometric Preliminaries 
    \begin{enumerate}
        \item BB localization 
        \item Intertwining functors and geometric fibers
        \item Lie algebra homology
    \end{enumerate}
    \item Lie algebra homology of standard Whittaker modules
    \item Contravariant Pairings 
    \begin{enumerate}
        \item definition
        \item classification
        \item generalization of Shapovalov form
        \item Radical of a pairing
    \end{enumerate}
    \item Costandard Whittaker modules
    \begin{enumerate}
        \item universal property
        \item algebraic definition 
        \item both algebraic and geometric definitions satisfy the universal property
    \end{enumerate}
    \item Whittaker modules form a highest weight category 
\end{enumerate}
